Data Insights as Data: Quick Overview and Exploration of Automated Data Insights

Automated data insight mining and visualization have been widely used in various business intelligence applications (e.g., market analysis and product promotion). However, automated insight mining techniques often output the same mining results to different analysts without considering their personal preferences, while interactive insight discovery requires significant manual effort. This paper fills the gap by integrating automated insight mining with interactive data visualization and striking a proper balance between them to facilitate insight discovery and exploration. Specifically, we regard data insights as a special type of data and further present InsightMap, a novel visualization approach that uses the map metaphor to provide a quick overview and in-depth exploration of different data insights, where a metric is proposed to measure the similarity between different insights. The effectiveness and usability of InsightMap are demonstrated through extensive case studies and in-depth user interviews.

==> src/10-conclusion.tex <==
\section{Conclusion} % and Future Work
In this paper, we proposed {\sysNameWithoutSpace}, an interactive visual analytics approach that combines automated insight extraction with interactive visual exploration to facilitate quick overview and in-depth exploration of automated data insights.
Specifically, we presented a generic quantitative technique to characterize each data insight (i.e., data insight embedding) and further measure the similarity between data insights.
Also, we introduced novel visualization designs using a metaphor of map to display the insight distribution as well as illustrate the relation (e.g., similarity) between data insights.
We further conducted extensive evaluations on our approach through three case studies on real datasets and carefully-designed user interviews with expert users. 
The evaluation results demonstrate the effectiveness and usability of our approach in assisting analysts with data insight exploration.
The lessons we learned and possible limitations are also explicitly discussed.

